PMNI: Pose-free Multi-view Normal Integration for Reflective and Textureless Surface Reconstruction

Reflective and textureless surfaces remain a challenge in multi-view 3D reconstruction. Both camera pose calibration and shape reconstruction often fail due to insufficient or unreliable cross-view visual features. To address these issues, we present PMNI (Pose-free Multi-view Normal Integration), a neural surface reconstruction method that incorporates rich geometric information by leveraging surface normal maps instead of RGB images. By enforcing geometric constraints from surface normals and multi-view shape consistency within a neural signed distance function (SDF) optimization framework, PMNI simultaneously recovers accurate camera poses and high-fidelity surface geometry. Experimental results on synthetic and real-world datasets show that our method achieves state-of-the-art performance in the reconstruction of reflective surfaces, even without reliable initial camera poses.

==> macro.tex <==
\newcommand{\gt}{GT\xspace}
\newcommand{\GT}{ground truth\xspace}
\newcommand{\drt}{DiLiGenRT\xspace}
\newcommand{\drts}{DiLiGenRT-S\xspace}
\newcommand{\dioo}{DiLiGenT\ensuremath{10^2}~\cite{ren2022diligent102}\xspace}
\newcommand{\dmv}{DiLiGenT-MV~\cite{li2020multi}\xspace}
\newcommand{\dd}{DiLiGenT~\cite{shi2019benchmark}\xspace}
\newcommand{\luces}{LUCES~\cite{logothetis2022cnn, mecca2021luces}\xspace}
\newcommand{\pss}{PS-SSS\xspace}
\newcommand{\ddp}{DiLiGenT-\ensuremath{\Pi}~\cite{wang2023diligent}\xspace}


% Method
\newcommand{\pmni}{PMNI\xspace}
\newcommand{\lsps}{LS~\cite{woodham1980ps}\xspace}
\newcommand{\pff}{PF14~\cite{papad14closed}\xspace}
\newcommand{\sdps}{SDPS-Net~\cite{chen2019self}\xspace}
\newcommand{\cnnps}{CNN-PS~\cite{ikehata2018cnn}\xspace}
\newcommand{\psfcn}{PS-FCN~\cite{chen2018ps}\xspace}
\newcommand{\stt}{ST14~\cite{shi2014bi}\xspace}
\newcommand{\attention}{NormAttention-PSN~\cite{ju2022normattention}\xspace}
\newcommand{\deconvn}{DeconvPS~\cite{inoshita2014surface}\xspace}
\newcommand{\thl}{TH28~\cite{shi2019benchmark}\xspace}
\newcommand{\thh}{TH46~\cite{shi2019benchmark}\xspace}
\newcommand{\msps}{MS-PS~\cite{hardy2022ms}\xspace}
\newcommand{\wgg}{WG10~\cite{wu2010robust}\xspace}
\newcommand{\pxnet}{PX-Net~\cite{logothetis2021px}\xspace}
\newcommand{\unips}{UniPS~\cite{ikehata2022universal}\xspace}
\newcommand{\sdmunips}{SDM-UniPS~\cite{ikehata2023scalable}\xspace}
\newcommand{\spline}{SPLINE-Net~\cite{zheng2019spline}\xspace}




